A Bayesian tune of the Herwig Monte Carlo event generator

The optimisation (tuning) of the free parameters of Monte Carlo event generators by comparing their predictions with data is important since the simulations are used to calculate experimental efficiency and acceptance corrections, or provide predictions for signatures of hypothetical new processes in experiments. We present a tuning procedure that is based on Bayesian reasoning and that allows for a proper statistical interpretation of the results. The parameter space is fully explored using Markov Chain Monte Carlo. We apply the tuning procedure to the Herwig7 event generator with both the cluster and the string hadronization models and a large set of measurements from hadronic Z-boson decays produced at LEP in $e^{+}e^{-}$ collisions. Furthermore, we introduce a coherent propagation of uncertainties from the realm of parameters to the realm of observables and we show the effects of including experimental correlations of the measurements. To allow comparison with the approaches of other groups, we repeat the tuning considering weights for individual measurements.

==> Makefile <==
#ulimit -u 10000
latexfile=BayesHerwigTune
newname?=BayesHerwigTune
STYLE=arxiv

LUALATEX=  export LANG="en_US.UTF-8";  lualatex
LATEX=  export LANG="en_US.UTF-8";  pdflatex -halt-on-error -shell-escape -enable-write18
BIBTEX=bibtex


ifeq ($(STYLE),draft)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-draft.tex lineno.sty mcite.sty units.sty
endif

ifeq ($(STYLE),arxiv)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-arxiv.tex mcite.sty units.sty
endif

ifeq ($(STYLE),jinst)
	STYLE_SPECIFIC_FILES=zeus_paper.cls $(latexfile)-jinst.tex mcite.sty units.sty jinstpub.sty JHEP.bst
endif

ifeq ($(STYLE),epjc)
	STYLE_SPECIFIC_FILES=svjour.cls  svepj.clo $(latexfile)-epjc.tex   
endif

#ifeq ($(STYLE),jhep)
#	STYLE_SPECIFIC_FILES=jheppub.sty $(latexfile)-jhep.tex JHEP.bst
#endif


all: $(latexfile)-$(STYLE).pdf


tables=


figures= \
Figures/H7_chisq_prob_all.pdf \
Figures/P8I_chisq_prob_all.pdf \
Figures/results_P8I.png \
Figures/P8I_chisq_prob_all_log.pdf \
Figures/results_H7.png \
Figures/compare_chisq_prob_all_log.pdf \
Figures/compare_chisq_prob_all.pdf \
Figures/H7_chisq_prob_all_log.pdf \
Figures/DELPHI_d15.pdf \
Figures/MULTI_d11.pdf \
Figures/H7_grid_pulls_skip_neg_respvals.pdf \
Figures/DELPHI_1996_S3430090-ClSmr-1-2.pdf \
Figures/DELPHI_1996_S3430090-ClPow-1-2.pdf \
Figures/DELPHI_1996_S3430090-AlphaQCD-1-2.pdf \
Figures/H7_fullruns_v5_assm013_cubic_pulls_positive_constr_redchi_full_basic.pdf \
Figures/DELPHI_1996_S3430090-ClMax-1-2.pdf \
Figures/P8I_weightone_chisq_prob_all.pdf \
Figures/H7_results_weighttwo.png \
Figures/H7_weightone_chisq_prob_all_log.pdf \
Figures/P8I_results_weighttwo.png \
Figures/H7_weightone_chisq_prob_all.pdf \
Figures/H7_weighttwo_chisq_prob_all_log.pdf \
Figures/H7_results_weightone.png \
Figures/P8I_weighttwo_chisq_prob_all_log.pdf \
Figures/P8I_results_weightone.png \
Figures/P8I_weighttwo_chisq_prob_all.pdf \
Figures/H7_weighttwo_chisq_prob_all.pdf \
Figures/P8I_weightone_chisq_prob_all_log.pdf \
Figures/sys_contour_P_ClMax__P_ClPow_.pdf \
Figures/P8_DELPHI_d15_log_MCvData_RD.pdf \
Figures/P8_MULTI_d11_MCvData_RD.pdf \
Figures/DELPHI_compare_log_MCvData_RD.pdf \
Figures/DELPHI_d15_log_MCvData_RD.pdf \
Figures/MULTI_compare_MCvData_RD.pdf \
Figures/MULTI_d11_MCvData_RD.pdf

arxiv-tar:
	tar -czvf arxiv.tar.gz $(latexfile)-arxiv.tex $(latexfile)-arxiv.bbl $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile).bib $(latexfile).bst $(latexfile)-fig.tex $(latexfile)-tab.tex Figures/ Tables/ mcite.sty units.sty zeus_paper.cls 

tar:  Makefile figurelist-$(STYLE).txt $(constanttables) $(tables)  $(latexfile)-def.tex  \
	$(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex  $(STYLE_SPECIFIC_FILES)
	rm -rf TAR
	mkdir -p TAR
	mkdir -p TAR/Figures
	#mkdir -p TAR/Tables
	cp Makefile   $(latexfile).bst $(latexfile).bib   $(latexfile)-def.tex $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex $(latexfile)-fig.tex    $(STYLE_SPECIFIC_FILES) TAR
	#cp $(tables) TAR/Tables
	for a in $$(cat   figurelist-$(STYLE).txt); do\
		cp $$a TAR/Figures;\
	done	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/*tex	
	sed -i 's@'$(latexfile)'@'$(newname)'@g' TAR/Makefile
	sed -i 's@^STYLE.*@STYLE='$(STYLE)'@g' TAR/Makefile
	
	sed -i 's@^Figures/tune_plots/@Figures/@g' TAR/Makefile
	sed -i 's@^Figures/error_prop/@Figures/@g' TAR/Makefile
	sed -i 's@^Figures/int_plots/@Figures/@g' TAR/Makefile
	sed -i 's@^Figures/weight_plots/@Figures/@g' TAR/Makefile
	sed -i 's@^Figures/correlation_plots/@Figures/@g' TAR/Makefile
	sed -i 's@^Figures/tuned_obs/@Figures/@g' TAR/Makefile
	
	sed -i '/@artic/achecked={2},'     TAR/*bib	
	sed -i '/@inproceed/achecked={2},' TAR/*bib	
	sed -i '/@phdthesis/achecked={2},' TAR/*bib	

ifeq ($(STYLE),epjc)
	sed -i 's@\[htbp\]@@g' TAR/$(latexfile)-tab.tex
	sed -i 's@c|@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@|c@c@g' TAR/$(latexfile)-tab.tex
	sed -i 's@}|@}@g' TAR/$(latexfile)-tab.tex
endif
	mv TAR/$(latexfile).bst TAR/$(newname).bst 
	mv TAR/$(latexfile).bib TAR/$(newname).bib 
#ifeq ($(STYLE),jhep)
#	rm TAR/$(newname).bst 
#endif
	mv TAR/$(latexfile)-$(STYLE).tex TAR/$(newname)-$(STYLE).tex
	mv TAR/$(latexfile)-txt.tex TAR/$(newname)-txt.tex
	mv TAR/$(latexfile)-abs.tex TAR/$(newname)-abs.tex
	mv TAR/$(latexfile)-tab.tex TAR/$(newname)-tab.tex
	mv TAR/$(latexfile)-def.tex TAR/$(newname)-def.tex
	mv TAR/$(latexfile)-fig.tex TAR/$(newname)-fig.tex
ifeq ($(STYLE),arxiv)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
ifeq ($(STYLE),jinst)
	#####-->A trick to get the bib file for axiv build system
	$(MAKE) -C TAR
	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
	$(MAKE) -C TAR clean
	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
endif
#ifeq ($(STYLE),jhep)
#	#####-->A trick to get the bib file for axiv build system
#	$(MAKE) -C TAR
#	mv TAR/$(newname)-$(STYLE).bbl  TAR/$(newname)-$(STYLE).bbl.temp
#	$(MAKE) -C TAR clean
#	cp TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname).bbl
#	mv TAR/$(newname)-$(STYLE).bbl.temp  TAR/$(newname)-$(STYLE).bbl
#endif

	tar -zcvf   $(newname).tar.gz -C TAR . 
	rm -rf $(newname).zip; cd TAR; zip ../$(newname).zip ./*/* ./*; cd ..
	#rm -rf TAR


       


$(latexfile)-$(STYLE).fls: $(constanttables) $(tables) \
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex   $(STYLE_SPECIFIC_FILES)
		pdflatex -recorder $(latexfile)-$(STYLE).tex
figurelist-$(STYLE).txt:  $(latexfile)-$(STYLE).fls
		cat $(latexfile)-$(STYLE).fls | grep pdf | grep Figures | sed 's@\./@@g' |sort | cut -f2 -d' '| uniq  > figurelist-$(STYLE).txt
		cat $(latexfile)-$(STYLE).fls | grep png | grep Figures | sed 's@\./@@g' |sort | cut -f2 -d' '| uniq  >> figurelist-$(STYLE).txt
constanttables=


$(latexfile)-$(STYLE).pdf :  $(figures) $(constanttables) $(tables) \
                    $(latexfile).bib $(latexfile)-abs.tex $(latexfile)-txt.tex $(latexfile)-tab.tex\
                     $(latexfile)-fig.tex  $(STYLE_SPECIFIC_FILES)
	
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
	$(BIBTEX) $(latexfile)-$(STYLE)
ifeq ($(STYLE),epjc)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
ifeq ($(STYLE),arxiv)
	sed -i 's@\\mbox{}.*@@g'  $(latexfile)-$(STYLE).bbl
endif
	$(LATEX) $(latexfile)-$(STYLE)
	$(LATEX) $(latexfile)-$(STYLE)


pdf : $(latexfile)-$(STYLE).pdf

$(latexfile).rws: $(latexfile)-dict.txt
	aspell --lang=en create master ./$(latexfile).rws < ./$(latexfile)-dict.txt

spell: $(latexfile).rws
		for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t \
			--add-tex-command="nospelling p" \
			--add-tex-command="prog p" \
			--add-tex-command="author p" \
			--add-tex-command="institute p" \
			--add-tex-command="text p" \
			--add-tex-command="affil  p" \
			--add-tex-command="Refrs p" \
			--dont-tex-check-comments -d en_US -c $$a ;\
		done

spelllist: $(latexfile).rws
		for a in $$(ls -1 $(latexfile)-*.tex); do\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		echo $$a;\
		echo "%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%" ;\
		aspell  --add-extra-dicts=./$(latexfile).rws  -t \
			--add-tex-command="nospelling p" \
			--add-tex-command="prog p" \
			--add-tex-command="author p" \
			--add-tex-command="institute p" \
			--add-tex-command="text p" \
			--add-tex-command="affil  p" \
			--add-tex-command="Refrs p" \
			--dont-tex-check-comments -d en_US list < $$a ;\
		done


clean :
	rm -f $(latexfile)-papers.tex
	rm -f *.aux
	rm -f *.lof
	rm -f *.out
	rm -f *.lot
	rm -f *.bbl
	rm -f *.l4l
	rm -f *.log
	rm -f *.blg
	rm -f *.ilg
	rm -f *.aux
	rm -f $(latexfile)*.dvi
	rm -f $(latexfile)*.ps
	rm -f $(latexfile)*.pdf
	rm -f *.toc
	rm -f *.idx
	rm -f *.ind
	rm -f *.nav
	rm -f *.snm
	rm -f *.rws

